Ftklipse - Design and Implementation of an Extendable Computer Forensics Environment: Specification Design Document

The purpose of this work is to design and implement a plugin-based environment that allows to integrate forensic tools working together to support programming tasks and addition of new tools. Integration is done through GUI components. The end-system environment must have user friendly GUI, configuration capabilities, plug-in capabilities to insert/inject new tools, case management, and chain of custody capabilities, along with evidence gathering capabilities, evidence preservation capabilities, and, finally report generation capabilities. A subset of these requirements has been implemented in Ftklipse, an open-source project, which is detailed throughout the rest of this document.

==> date.tex <==
Fri 12 Jun 2009 19:44:34 EDT

